Why We Engage in FLOSS: Answers from Core Developers

The maintenance and evolution of Free/Libre Open Source Software (FLOSS) projects demand the constant attraction of core developers. In this paper, we report the results of a survey with 52 developers, who recently became core contributors of popular GitHub projects. We reveal their motivations to assume a key role in FLOSS projects (e.g., improving the projects because they are also using it), the project characteristics that most helped in their engagement process (e.g., a friendly community), and the barriers faced by the surveyed core developers (e.g., lack of time of the project leaders). We also compare our results with related studies about others kinds of open source contributors (casual, one-time, and newcomers).

==> sections/discussion.tex <==
\begin{table*}[!t]
	\centering
	\caption{Comparison of our findings by project size and GitHub account.}
	\small
	\begin{tabularx}{\textwidth}{ @{}l | l | r | r | r | r@{}}
		\toprule
		\multicolumn{1}{c|}{\bf Topic}  					& \multicolumn{1}{c|}{\bf Top-3 reasons}  																				& \multicolumn{1}{r|}{\bf User}								& \multicolumn{1}{r|}{\bf Organization}							& \multicolumn{1}{r|}{\bf Small-Medium} 							& \multicolumn{1}{r}{\bf Medium-Large}\\ 	 
		\midrule
		\begin{tabular}[c]{@{}l@{}} Motivations\end{tabular}			& \begin{tabular}[c]{@{}X@{}}\\[-.25cm]To improve the project because I am using it\\\\[-.25cm] To have a volunteer work\\\\[-.25cm] I have interest or expertise on the project domain\end{tabular} 	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]11\%\\\\[-.25cm]-15\%\\\\[-.25cm]-6\%\end{tabular}	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-11\%\\\\[-.25cm]15\%\\\\[-.25cm]6\%\end{tabular}	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]6\%\\\\[-.25cm]-13\%\\\\[-.25cm]-4\%\end{tabular}		& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-6\%\\\\[-.25cm]13\%\\\\[-.25cm]4\%\end{tabular}	\\
		\hline
		\begin{tabular}[c]{@{}l@{}} Project\\characteristics \end{tabular} 	& \begin{tabular}[c]{@{}X@{}}\\[-.25cm]Friendly community\\\\[-.25cm]Availability of the project leaders\\\\[-.25cm]Unit tests  \end{tabular}								& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-12\%\\\\[-.25cm]2\%\\\\[-.25cm]10\%\end{tabular}	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]12\%\\\\[-.25cm]-2\%\\\\[-.25cm]-10\%\end{tabular}	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-17\%\\\\[-.25cm]-15\%\\\\[-.25cm]12\%\end{tabular} 	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]17\%\\\\[-.25cm]15\%\\\\[-.25cm]-12\%\end{tabular} 	\\
		\hline
		\begin{tabular}[c]{@{}l@{}} Barriers \end{tabular} 			& \begin{tabular}[c]{@{}X@{}}\\[-.25cm]Lack of time of project leaders\\\\[-.25cm] Large and complex project\\\\[-.25cm] Unclear, complex or buggy code \end{tabular}					& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]3\%\\\\[-.25cm]-35\%\\\\[-.25cm]5\%\end{tabular}		& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-3\%\\\\[-.25cm]35\%\\\\[-.25cm]-5\%\end{tabular}	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]30\%\\\\[-.25cm]-18\%\\\\[-.25cm]-13\%\end{tabular} 	& \begin{tabular}[r]{@{}r@{}}\\[-.25cm]-30\%\\\\[-.25cm]18\%\\\\[-.25cm]13\%\end{tabular}	\\
		\bottomrule
	\end{tabularx}
	\label{tab:comparison-by-project-size-and-github-account}
\end{table*}

Many popular GitHub projects have a low (one or two) bus factor~\cite{avelino2016novel}, i.e.,~face the risk of key personnel leaving the project.
Ye and Kishida~\cite{ye2003toward} find that development of GIMP was once halted because a key core developer left the project.
Therefore, FLOSS projects must attract new core developers to share the maintenance and knowledgement to mitigate the risks of failure.
However, the developers who participated of our survey contribute for different kinds of projects (e.g.,~small and larger projects, and projects ran by companies and by individuals), which can present some differences on their motivations to contribute and the barriers faced by them.
For example, developers who contribute to a small projects maybe not have complication with the complexity of the project.
For this reason, we conduct a segmented analysis of the survey answers in two groups: (i) groups associated to project size in terms of LOC and (ii) groups associated to GitHub account type.
First, we calculate the percentage of all 52 survey answers for individual account (34.6\%) and for organization account (65.4\%) and also the percent for small (32.7\%) and large projects (67.3\%).
Then, we calculate the percentage for these groups for each Top-3 survey answers for motivations, project characteristics and barriers.
For example, the motivation ``To improve the project because I am using it'' have 45.2\% of answers for individual and 54.8\% for organization account, and 38.7\% for small and 61.3\% for large projects.
In the next step, we calculate the difference of these percentages. As example, the difference for individual measure 11\% (45.2\% - 34.6\%) and for organization account measure -11\% (54.8\% - 65.4\%), and 
for small is 6\% (38.7\% - 32.7\%) and for large projects is -6\% (61.3\% - 67.3\%).
So, the goal of this analysis is identify if the motivations to contribute and the barriers are influenced by GitHub account or the size of the project.
Table~\ref{tab:comparison-by-project-size-and-github-account} summarizes the segmented analysis for the Top-3 survey answers for the motivations, project characteristics and practices, and the barries faced by the developers.

\noindent{\bf Groups associated to project size in terms of LOC:}

\noindent{\bf Groups associated to GitHub account type:} 

==> sections/surveyDesign.tex <==
In this study, we start by considering the top-5,000 most popular GitHub projects ranked by their number of stars. Then, we apply four strategies to discard projects, as follows: 

\begin{itemize}
\item \textit{Non-Software Projects} - We discarded 61 repositories from our initial list that are not software systems. Specifically, we prune projects like books (e.g., {\sc vhf/free-programming-books} and {\sc getify/You-Dont-Know-JS}) and awesome-list (e.g., {\sc sindresorhus/awesome}). 
\item \textit{Projects with no LOC} - We set the tool {\sc AlDanial/cloc} up to consider programming languages according to Tiobe list\footnote{https://www.tiobe.com/tiobe-index//}. In this filter, we discarded 397 projects with the number of LOC equal to zero. As an example, we removed from our list {\sc github/gitignore}, {\sc jlevy/the-art-of-command-line}, and {\sc necolas/normalize.css}.
\item \textit{Period of Idleness} - We are interested in projects that have reached stable states and are being actively developed. Therefore, we discarded 830 repositories without commits in the last six months.
\item \textit{New Repositories} - In this study, we consider the repository creation date to focus on stable projects. For this reason, we discarded 1,450 repositories which are forks or have less than three years. 
\end{itemize}


\begin{table}[!ht]
\centering
\caption{Strategies used to filter out projects to create the dataset}
\begin{tabular}{ l r l }
\toprule
{\bf Strategy}			& \multicolumn{2}{c}{\bf \# Discarded Projects}	\\ 
\midrule
Non Software Projects		& 61 	& \sbar{61}{\totalRemovedSystem} \\
Computation of LOC		& 397 	& \sbar{397}{\totalRemovedSystem} \\
Period of Idleness		& 830	& \sbar{830} {\totalRemovedSystem} \\
New Repositories		& 1,450	& \sbar{1450} {\totalRemovedSystem} \\
\bottomrule
Total of Discarded Projects 	& 2,738 & \\
\bottomrule
\end{tabular}
\label{tab:Filters}
\end{table}


%First, we selected the top-5,000 most popular projects on GitHub, using the number of stars as a proxy for popularity. From this initial list, we removed 1,695 repositories which are forks or have less than three years considering the creation date of the repository, to focus the study on mature projects. We also discarded 1,005 repositories without commits in the last six months.

Table~\ref{tab:Filters} summarizes the number of removed projects to create our dataset. Some discarded projects are on the top-10 from our initial list, e.g., {\sc vhf/free-programming-books} (95,414 stars), {\sc getify/You-Dont-Know-JS} (68,484 stars), and {\sc github/gitignore} (55,517 stars). 
We ended up with a list of 2,262 systems, including well-known projects, like {\sc facebook/react}, {\sc angular/angular}, and {\sc rails/rails}. 


Figure~\ref{dataset_violinplot_projects_characteristics} shows violin plots with the distribution of age (in months), number of contributors, number of commits, and number of stars of the selected projects, without considering outliers. 
The median measures are 59 months, 50 contributors, 826 commits, and 3.1K stars, respectively. 
1,256 projects (55\%) are owned by organizations and 1,006 repositories (45\%) by users. 
The projects are implemented in JavaScript (696 projects, 31\%), followed by Ruby (232 projects, 10\%), and Python (230 projects, 10\%).

\begin{figure*}[!t]
  \centering
\subfloat[ref1][Age]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_age}}
\quad
\subfloat[ref2][Contributors]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_contributors}}
\quad
\subfloat[ref3][Commits]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_commits}}
\quad
\subfloat[ref4][Stars]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_stars}}
\caption{Distribution of the (a) age, (b) contributors, (c) commits, and (d) stars of the selected projects, without considering outliers.}
\label{dataset_violinplot_projects_characteristics} 
\end{figure*}

\begin{figure*}[!t]
  \centering
\subfloat[ref1][Core team contributions]
{
\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_percent_contributions}
}
\quad
\subfloat[ref2][Core team size]
{
\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_core_team_size_with_threshold}
}
\quad
\subfloat[ref3][Core developer contributions]
{
\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_percent_of_core_contributors_with_threshold} 
}
\caption{(a) Total percentage of commits by the selected core teams, (b) number of core developers per project, and (c) percentage of commits by the selected core developers.
Outliers are ommited in all violin plots.}
\label{percent_of_contributions}
\end{figure*}

\subsection{Core Developer Identification}

We identified the core developers for each project using a Commit-Based Heuristic, which is commonly adopted in other works~\cite{mockus2002two, robles2009evolution, dinh2005freebsd, koch2002effort}. 
The heuristic is centered on the number of commits by developers which follows a heavy-tailed distribution~\cite{mockus2002two,koch2002effort}, i.e., a minority of developers accounts for most contributions.  
The goal is to identify the core team as those who produce 80\% of the overall amount of commits in a project. 
However, the core team can contains developers with few contributions in relation to the total number of commits. 
%The algorithm consists of the following steps: In the first step, the algorithm counts how many commits each developer applied. After that, the developers are sorted by descending order according to their number of commits. Finally, the algorithm selects the first developers 
For this reason, we customized this heuristic to require that a core developer must have at least 5\% of the total number of commits; thus, candidates who have few commits are excluded. 
After applying this threshold, the core team may not achieve 80\% of the total number of commits.
For example, to achieve around 80\% of the commits in {\sc mrdoob/three.js}, the core team identified by the heuristic consists of 11 contributors.
However, nine contributors have less than 5\% of the overall amount of commits. Thus, only two developers are classified as \textit{core} by our customized heuristic.
These developers represent 55\% and 10\% of the project's commits, respectively.

Despite of this new threshold, we can observe in Figure~\ref{percent_of_contributions}a that the median percentage of commits by the selected core teams is 81\%.
Figure~\ref{percent_of_contributions}b shows the core team size per project considering the commit minimal threshold of 5\%. 
As presented in Figure~\ref{percent_of_contributions}c, the median percentage of commits by the core developers identified with the adapted heuristic is 19\%, in contrast to the original strategy (0.5\%).


%However, we also customized this heuristic to require that a core developer must have at least 5\% of the total number of commits, to exclude candidates who have few commits.
%Therefore, after applying this threshold, the core team may not achieve 80\% of the total number of commits. For example, to achieve around 80\% of the commits in {\sc mrdoob/three.js}, the core team would be composed by 11 contributors. Nevertheless, nine contributors have less than 5\% of the total number of commits and only two developers are then considered core by our customized heuristic. These developers represent 55\% and 10\% of the projects' commits, respectively. Despite the application of this threshold, the median number of commits by the selected core teams is 81\%, as showed in Figure~\ref{percent_of_contributions}a. In Figure~\ref{percent_of_contributions}b, we show the core team size per project considering the minimal threshold of 5\% of the commits. As presented in Figure~\ref{percent_of_contributions}c, the median percentage of commits by the core developers selected by our heuristic is 19\%, against only 0.5\% when the proposed threshold is not in place.

Finally, we follow three steps for each project to select the core developers:

\begin{itemize}
	\item We apply the adapted heuristic on all commits of the project (set A).
	\item We remove the last year of commits and calculate again the core team (set B).
	\item The selected set of {\em core developers} is formed by developers in the set A, but who are not in B. In other words, this group includes developers who have entered in the core team last year.
\end{itemize}

We ended up with a list of 380 new core developers who are distributed over 331 projects.

\subsection{Survey Design}
\label{subsec:survey_design}

%We conducted a survey with the identified developers to understand what motivated them to become a core member and the main barriers they faced during the process.

We conducted a survey to search for the rationale behind the identified developers' motivation to become a core member and the main barriers they faced during the process. 
%Both surveys took place in two rounds, a pilot round that gave us the opportunity to field test our initial questions and the final round with some adjusts.
After removing the core developers who do not have a public e-mail address on GitHub, we obtained a list of 151 potential participants. 
Figure~\ref{fig:emailTemplate} shows the template of our survey email sent to these developers. The survey email is planned with two parts: First, we customized the survey email to include the developer's name (line one) and the project name (line four). Then, the second part presents  three open-ended questions (lines 8---9) related to his/her contributions for the project: (1) What motivated you to contribute on this project? (2) Which project characteristics and practices helped you to contribute? (3) What were the main barriers you faced to cooperate?  


%\begin{enumerate}
%\item What motivated you to contribute to the project?
%\item Which project characteristics and practices helped you to contribute?
%\item Which were the main barriers you faced to contribute?
%\end{enumerate}


\begin{figure}[!h]
\begin{center}
\begin{lstlisting}[linewidth=\columnwidth,breaklines=true]
Dear <Name>, 

I'm ... investigating strategies for sustaining open-source projects. I found that you have become one of the main developers for the <Project Name>, with xx % of the project's commits.

Could you please answer three questions about your contributions to this project?

1. What motivated you to contribute on this project?
2. What project characteristics and practices helped you to contribute?
3. What were the main barriers you faced to cooperate?

\end{lstlisting}
\caption{E-mail template of the survey sent to developers of the selected projects}
\label{fig:emailTemplate}
\end{center}
\end{figure}

We collected 52 answers out of 151 survey emails sent to developers (response rate of 34\%). 
Then, we organized the responses into groups to conduct our analysis, as follows: 

\paragraph{(i) Groups associated to project size in terms of LOC} We classified the 52 projects related to developers---who answered the survey---into Small and Large projects. The projects in the first and second quartiles are assigned as Small, and the third and fourth quartiles as Large, with 17 and 35 projects, respectively. 
Figure~\ref{fig:files_loc}a shows the number distribution of files for selected projects with the first (X), median (44), and third (X) quartile measures. The violin plot in Figure~\ref{fig:files_loc}b describes the size of these files in LOC. The first, median, third quartiles are X, 4,9k, and Y, respectively.
 

\paragraph{(ii) Groups associated to GitHub account type} We inspected each project account and organized 
in Individual and Organizational accounts, with 18 and 34 projects, respectively.

\begin{figure}[!h]
  \centering
%\vspace{1mm}
\subfloat[ref1][Files]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_files}}
\quad
\subfloat[ref2][LOC]{\includegraphics[width=\lenghtFigure \textwidth]{Figures/violinplot_loc}}
\caption{Distribution of the (a) number of files and (b) LOC of the projects, both violin plots without outliers.}
\label{fig:files_loc}
\end{figure}



Finally, we use Thematic Analysis~\cite{cruzes2011recommended} to interpret the survey answers. 
This technique is used for identifying and recording ``themes'' (i.e., patterns) in textual documents. 
In summary, Thematic Analysis consists of: (1) identifying themes from the answers, (2) reviewing the themes to find patterns for merging, and (3) defining and naming the final themes. 
First, the initial theme identification and merge steps were performed independently by each author of this paper. 
Then, we had some meetings to resolve conflicts and to define the final themes. 
In the first question, both authors suggested semantically equivalent themes for 32 answers (62\%). 
Therefore, these themes were then rephrased and standardized to compose the final theme set. 
As the remaining 20 answers had divergent themes, they were discussed by both authors to reach a consensus.
For the last two questions, an initial agreement was reached in 36 (69\%) and 38 (73\%) answers, respectively.
%In 31 (65\%), 35 (73\%), and 37 (77\%) cases for questions one, two, and three, respectively, both authors suggested semantically equivalent themes that were rephrased and standardized to compose the final set of themes. 
%The remaining answers with divergent themes were then discussed by both authors to reach a consensus.
%In 94 cases (35\%), one author accepted the theme proposed by the other author. 
%In the remaining 18 cases (7\%), the final theme emerged from the discussion and was different from what both authors previously suggested.
